Entity Resolution with Empirically Motivated Priors

Databases often contain corrupted, degraded, and noisy data with duplicate entries across and within each database. Such problems arise in citations, medical databases, genetics, human rights databases, and a variety of other applied settings. The target of statistical inference can be viewed as an unsupervised problem of determining the edges of a bipartite graph that links the observed records to unobserved latent entities. Bayesian approaches provide attractive benefits, naturally providing uncertainty quantification via posterior probabilities. We propose a novel record linkage approach based on empirical Bayesian principles. Specifically, the empirical Bayesian--type step consists of taking the empirical distribution function of the data as the prior for the latent entities. This approach improves on the earlier HB approach not only by avoiding the prior specification problem but also by allowing both categorical and string-valued variables. Our extension to string-valued variables also involves the proposal of a new probabilistic mechanism by which observed record values for string fields can deviate from the values of their associated latent entities. Categorical fields that deviate from their corresponding true value are simply drawn from the empirical distribution function. We apply our proposed methodology to a simulated data set of German names and an Italian household survey, showing our method performs favorably compared to several standard methods in the literature. We also consider the robustness of our methods to changes in the hyper-parameters.

==> sec4-point-estimate-v24.tex <==
\section{Estimated Linkage Structure}
\label{sec:linkage-structure}
Using the Gibbs samples, we can easily compute the posterior probability that any set of records match.
%, i.e., that they refer to the same individual.  
However,
we may wish to report a single
estimate of the entire linkage structure, since this is often more meaningful.
The application of a simple pairwise thresholding rule (e.g., estimate that two records are linked if and only if their posterior matching probability exceeds $1/2$) can produce an estimated linkage structure that is non-transitive.  For example, it is possible for the posterior matching probability to exceed $1/2$ for record pairs A--B and B--C but not for record pair A--C.  Then the resulting estimated linkage structure would claim that records A and~B are the same individual, and that records B and~C are the same individual, while records A and~C are \emph{not} the same individual.  Clearly such an estimate is nonsensical.

Thus, some care is necessary to construct an estimate that avoids the aforementioned problem, i.e., that preserves transitivity.  We follow the framework for constructing such an estimate that was laid out by \citet{steorts_2013b}, which we now describe.
%  which caries through precisely over to the framework that we have constructed.
%  Two records $(i_1,j_1)$ and $(i_2,j_2)$ {\em match} if they
%point to the same latent individual, hence the 
%rior probability of a match can be computed from the $S_G$ MCMC
%samples:
%$
%P(\lambda_{i_1j_1} = \lambda_{i_2j_2} | \bm{X}) = \frac{1}{S_G}\sum_{h=1}^{S_G}
%I(\lambda_{i_1j_1}^{(h)} = \lambda_{i_1j_2}^{(h)}).$ 
First, for any particular linkage structure, each record's \emph{maximal matching set} (MMS) is simply the set of records that are linked to the same latent individual as the record in question.  The posterior probabilities of the various possible linkage structures thus imply posterior probabilities that various sets of records are the MMS for a particular record.  Each record's \emph{most probable maximal matching set} (MPMMS) is the set with the highest posterior probability of being the MMS for that record.
Finally, a set of records is a \emph{shared most probable MMS} if it is the most probable MMS for each record that it contains.
Then the overall estimated linkage structure is constructed by linking records if and only if they are members of the same shared most probable MMS.
This procedure is guaranteed to preserve transitivity since each record can be a member of no more than one shared most probable MMS. Furthermore,  any record that is not a member of \emph{any} shared most probable MMS is simply not linked to any other record.

==> sec5-divergence-v30.tex <==
\section{Theoretical Properties of Record Linkage}


We next derive bounds for the tail probabilities of the distribution of errors in the regarding the linkage structure 
under the model of \cite{steorts_2013b}. We are able to show when the latent individuals become more distinct and more similar. Then under our proposed model, we derive a lower bound on recovering the corrupted data that depends on a moment generating function. Furthermore, the rate of recovering the data is dependent on the same moment generating function of the distance between one of the latent entities and a realization $m$.


In Shannon entropy or minimax theory, we often seek to know if some signal $Y$ can be recovered from the received signal $X$ in the presence of some noise $z.$ This often occurs in the signal processing literature. Suppose $\hat{Y}$ is not quite $Y$ but we allow some decoding or reconstruction error.
%Then what conditions must hold for $X$ or $z$ or $Y?$
We propose exploring this through minimax theory and  Kullback-Leibler (KL) divergence to understand the difference between the perturbed distributions of $\bX$ when two latent individuals are not the same.

Recall the connection to Kullback-Leibler (KL) divergence in the sense that for any two distributions $P$ and $Q$, the maximum power for testing $P$ versus $Q$ is $\exp\{-n D_{\text{KL}}(P || Q)\}.$ Hence, low $D_{KL}$ means we need many samples to distinguish $P$ from $Q.$  How then does changing $\bY$ or $\lam$ change the distribution of $\bX?$ We search for both meaningful upper and lower bounds since an upper bound will say that $P$ and $Q$ are never more than so far apart, whereas a lower bound says how easy it is to tell $P$ and $Q$ apart. 

\subsection{KL Divergence Bounds}
We investigate how well can we recover $\bY$ and $\lam$ from $\bX.$ For any two distributions $P$ and $Q$, the maximum power for testing $P$ versus $Q$  \citep{kullback_1951}
 is $$O(\exp\{- N \; D_{\text{KL}}(P || Q)\}).$$ Hence, low $D_{\text{KL}}$ means it is intrinsically hard to tell $P$ from $Q.$



Let $P = f(X\mid \bY, \lam, \bm{\theta}, \bm{\beta})$ and $Q=
 f(X\mid \bY^\prime, \lam^\prime, \bm{\theta}, \bm{\beta}).$
%
We know that $X_1,X_2,\ldots,X_N$ are all independent given $(\bY,\lam, \bm{\theta}, \bm{\beta})$ under both $P$ and $Q.$ This implies that 
$$D_{X_1, X_2, \ldots, X_N} (P \| Q) = \sum_i D_{X_i}(P \| Q).$$

\subsubsection{KL Divergence under Categorical Data}

We assume the model of \cite{steorts_2013b}, which assumes that data is categorical. Under the same notation previously used, we simply recall the model under categorical data of these papers. 

\citet{steorts_2013b} assume the $k$ files are conditionally independent given the latent
individuals, and that fields are independent within individuals. We assume that model (\ref{mod:hb}) holds in Section \ref{sec:hb}. 
%\begin{align*}
%\bm{x}_{ij\ell}\mid\lambda_{ij},\bm{y}_{\lambda_{ij}\ell},z_{ij\ell},\bm{\theta}_\ell&\stackrel{\text{ind}}{\sim}
%\begin{cases}
%\delta_{\bm{y}_{\lambda_{ij}\ell}}&\text{ if }z_{ij\ell}=0\\
%\text{MN}(1,\bm{\theta}_\ell)&\text{ if }z_{ij\ell}=1
%\end{cases}\\
%z_{ij\ell}&\stackrel{\text{ind}}{\sim}\text{Bernoulli}(\beta_\ell)\\
%\bm{y}_{j'\ell}\mid\bm{\theta}_{\ell}&\stackrel{\text{ind}}{\sim}\text{MN}(1,\bm{\theta}_\ell)\\
%\bm{\theta}_\ell&\stackrel{\text{ind}}{\sim}\text{Dirichlet}(\bm{\mu}_\ell)\\
%\beta_\ell&\stackrel{\text{ind}}{\sim}\text{Beta}(a_\ell,b_\ell) \\
%\pi(\lam) &\propto 1,
%\end{align*}
%where
%$a_\ell,b_\ell,$ and $\bm{\mu}_\ell$ are all known.
Consider $f(X\mid \bY, \lam, \bm{\theta}, \bm{\beta}). $ Then
\begin{align*}
Pr(X_{ij\ell} =m \mid \bY, \lam, \bm{\theta}, \bm{\beta})
&= 
Pr(X_{ij\ell} =m, Z_{ij\ell} = 0 \mid \bY, \lam, \bm{\theta}, \bm{\beta}) \\
&+ Pr(X_{ij\ell} =m, Z_{ij\ell} = 0 \mid \bY, \lam, \bm{\theta}, \bm{\beta})\\
&= Pr(X_{ij\ell} =m \mid \bY, \lam, \bm{\theta}, \bm{\beta}, Z_{ij\ell} = 1) 
Pr( Z_{ij\ell} = 1 \mid  \bY, \lam, \bm{\theta}, \bm{\beta})\\
&+ Pr(X_{ij\ell} =m \mid \bY, \lam, \bm{\theta}, \bm{\beta}, Z_{ij\ell} = 0) 
Pr( Z_{ij\ell} = 0 \mid  \bY, \lam, \bm{\theta}, \bm{\beta})\\
&= 1(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) 
+ \theta_{\ell m} \beta_{\ell}.
\end{align*}
Then $$D_{X_{ij\ell}}(P\| Q) = \sum_{m=1}^{M_\ell} 
\{
I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}\}
\log\left[
\frac{I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}}
{
I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}
}
\right].$$
This implies
$$D_{\bX} (P\| Q) =
\sum_{ij\ell m} \left\{
I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}\}
\log\left[
\frac{I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}}
{
I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}
}
\right]
\right\}.$$

Let $t_{ij\ell} = Y_{\Lambda_{ij}\ell} $ and 
$t^\prime_{ij\ell} = Y^\prime_{\Lambda^\prime_{ij}\ell}. $

Note that \textcolor{black}{if $t_{ij\ell} \neq t^{\prime}_{ij\ell}$}, then
\begin{align*}
\| P-Q\|_1 &= \sum_m \left | I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}
-I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) (1-\beta_{\ell}) -  \theta_{\ell m} \beta_{\ell}
\right | \\
&= \sum_m \left | I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) -I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) (1-\beta_{\ell})   
\right | \\
&= 2(1-\beta_\ell)
\end{align*}
since $P(m) = Q(m)$ unless $m = t_{ij\ell}$ or $m = t^\prime_{ij\ell}.$
\textcolor{black}{If $t_{ij\ell} = t^{\prime}_{ij\ell}$, then $P=Q$ and $\|P-Q\|_1 = 0$.}
%
The reverse Pinsker inequality of \cite{berend_2014} relates the KL
divergence to the $L_1$ norm in the following way:
$D(P \| Q) \leq \| P-Q\|_1 \ln \{ (\min Q)^{-1}\}.$ Using this, we find that \textcolor{black}{(if $t_{ij\ell} \neq t^{\prime}_{ij\ell}$)}
\begin{align*}
D(P \| Q) &\leq 2(1-\beta_{\ell}) \ln \left \{
\dfrac{1}{
\min_m I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) (1-\beta_{\ell}) +  \theta_{\ell m} \beta_{\ell}
}
\right\}\\ 
&\leq 
2(1-\beta_{\ell}) \ln \left \{
\dfrac{1}{
\min_m \theta_{\ell m} \beta_{\ell}
}
\right\}.
\end{align*}
Hence, $D_{\bX}(P \| Q)\leq 
2\sum_{ij\ell} I(t_{ij\ell} \neq t^{\prime}_{ij\ell}) (1-\beta_{\ell}) \ln \left \{
\dfrac{1}{
\min_m \theta_{\ell m} \beta_{\ell}
} 
\right\}:=\gamma.$ 
%
Using Fano's inequality, we find that the minimum probability of getting a latent individual wrong is
$$Pr( (\hat{\lam}, \by) \ne (\lam, \by)) \geq 1 - \frac{ \gamma + \ln 2}{\ln r},$$ where $r+1$ is the number of 
$(\lam, \by)$ pairs. That is, as the latent individuals become more distinct, $\gamma$ increases. On the other hand, as the latent individuals become more similar, $\gamma \rightarrow 0.$

\begin{rem}
Suppose $\beta_{\ell} \rightarrow 1.$ Then the bound reduces to $D_{\bX}=0.$ This implies that when there is growing distortion, there is no difference between two latent individuals. Suppose $\beta_{\ell} \rightarrow 0.$ Then the upper bound is infinite, which is not informative here. 
\end{rem}

Using Pinsker's  inequality,
\begin{align*}
D(P \| Q) \geq \dfrac{1}{4}||P-Q||^2_1
&\implies D(P \| Q) \geq I(t_{ij\ell} \neq t^{\prime}_{ij\ell}) (1-\beta_{\ell})^2 \\
&\implies
D_{\bX}(P \| Q) \geq \sum_{ij\ell} I(t_{ij\ell} \neq t^{\prime}_{ij\ell})  (1-\beta_{\ell})^2.
\end{align*}

\begin{rem}
Suppose $\beta_{\ell} \rightarrow 1.$ Then $D_{\bX} \geq 0.$ If instead $\beta_{\ell} \rightarrow 0,$ then $D_{\bX} \geq 1.$ The lower bound is only informative when $\beta_{\ell} \rightarrow 0.$ We have more information when the latent individuals are separated.
\end{rem}

\subsection{K-L Divergence Bounds for String and Categorical Data}
We now consider $P$ and $Q$ under the EB model proposed in this paper for both categorical and non-categorical data. We find that
\begin{align*}
Pr(X_{ij\ell} =m \mid \bY, \lam, \bm{\theta}, \bm{\beta})
&= 
Pr(X_{ij\ell} =m, Z_{ij\ell} = 0 \mid \bY, \lam, \bm{\theta}, \bm{\beta}) \\
&+ Pr(X_{ij\ell} =m, Z_{ij\ell} = 0 \mid \bY, \lam, \bm{\theta}, \bm{\beta})\\
&= Pr(X_{ij\ell} =m \mid \bY, \lam, \bm{\theta}, \bm{\beta}, Z_{ij\ell} = 1) 
Pr( Z_{ij\ell} = 1 \mid  \bY, \lam, \bm{\theta}, \bm{\beta})\\
&+ Pr(X_{ij\ell} =m \mid \bY, \lam, \bm{\theta}, \bm{\beta}, Z_{ij\ell} = 0) 
Pr( Z_{ij\ell} = 0 \mid  \bY, \lam, \bm{\theta}, \bm{\beta})\\
&\propto I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) 
+ \alpha_{\ell } (X_{ij\ell})\beta_{\ell} \bigg[ 
\exp \{
-c\;d(X_{ij\ell}, Y_{\lambda_{ij}\ell})
\}
\bigg].
\end{align*}
Suppose that $t_{ij\ell} \neq t^{\prime}_{ij\ell}$ (as otherwise the divergence between $P$ and $Q$ is trivially~$0$).  Then 
\hspace*{-5em}
\begin{align*}
D_{X_{ij\ell}}(P\| Q)
&\propto \sum_{m=1}^{M_\ell} 
I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) 
+ \alpha_{\ell } (m)\beta_{\ell}  \times
%\bigg[ 
e^{
-c\;d(X_{ij\ell}, Y_{\lambda_{ij}\ell}) 
} \times \\
%\bigg]
& \qquad \log\left[
\frac{
I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) 
+ \alpha_{\ell } (m)\beta_{\ell} \bigg[ 
e^{
-c\;d(m, Y_{\lambda_{ij}\ell})
}
\bigg]
}
{
I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) (1-\beta_{\ell}) 
+ \alpha_{\ell } (m)\beta_{\ell} \bigg[ 
e^{
-c\;d(m, Y^{\prime}_{\lambda^\prime_{ij}\ell})
}
\bigg]}
\right].
\end{align*}
Note that 
\begin{align*}
\| P-Q\|_1 &= \sum_{m\in M_\ell}\left| I(Y_{\Lambda_{ij}\ell} = m) (1-\beta_{\ell}) + \alpha_\ell(m) \beta_{\ell}
 \exp \{
-c\;d(m, Y_{\lambda_{ij}\ell}^{})
\}
\right.\\
&\left.\qquad\qquad -
I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) (1-\beta_{\ell}) - \alpha_\ell(m)  \beta_{\ell}
 \exp \{
-c\;d(m, Y^\prime_{\lambda^\prime_{ij}\ell})
\}\right|.
\end{align*}
We can show that 
\begin{align*}
\| P-Q\|_1
 &\leq 
 \sum_m  (1-\beta_{\ell})\left | \left[I(Y_{\Lambda_{ij}\ell} = m) -I(Y^\prime_{\Lambda^\prime_{ij}\ell} = m) \right] \right|\\
 &+ \sum_m  \alpha_\ell(m)  \beta_{\ell}
 \left| 
 \exp\{
 -c\; d(m, Y_{\lambda_{ij}\ell})
 -
  \exp\{
 -c\; d(m, Y^\prime_{\lambda^\prime_{ij}\ell})
 \}\right| \\
 & \leq 2 (1- \beta_\ell) + \beta_\ell \sum_m \alpha_\ell(m) 
  \left| 
 \exp\{
 -c\; d(m, Y_{\lambda_{ij}\ell})
 -
  \exp\{
 -c\; d(m, Y^\prime_{\lambda^\prime_{ij}\ell})
 \} \right|.
\end{align*}
Suppose the two field attributes are different. That is, there exists an $m \neq m^\prime.$ Then we assume that there exists a $\delta >0 $ such that $d(m,m^\prime) \geq \delta.$ Then 
we write 
\begin{align*}
\| P-Q\|_1
 & \leq 2 (1- \beta_\ell) + \beta_\ell \sum_m \alpha_\ell(m) 
  \left| 
 \exp\{
 -c\; d(m, Y_{\lambda_{ij}\ell})
 -
  \exp\{
 -c\; d(m, Y^\prime_{\lambda^\prime_{ij}\ell})
 \} \right|.
\end{align*}
By the reverse triangle inequality, for any $m, m^\prime, m^{\prime \prime},$
\begin{align*}
| d(m, m^\prime) - d(m, m^ {\prime \prime}) |
&\leq d(m^\prime, m^ {\prime \prime}) \implies
e^{-c [  d(m, m^\prime) -d(m, m^ {\prime \prime}) ] }
& \geq
e^{-c d(m^\prime, m^ {\prime \prime}) },
\end{align*}
which in turn implies that
\begin{align*}
&\sum_m \left[
\left(1 - e^{-c [  d(m, m^\prime) - d(m, m^ {\prime \prime}) ] }\right)
e^{-c d(m^\prime, m^ {\prime \prime}) } \alpha_\ell (m)
\right]\\
& \qquad
\sum_m
\left(1 - e^{-c [ d(m^\prime, m^ {\prime \prime}) ] }\right) 
e^{-c d(m^\prime, m^ {\prime \prime}) } \alpha_\ell (m).
\end{align*}
Then 
\begin{align*}
\sum_m  \alpha_\ell (m)
\left[
e^{-c  d(m, m^\prime)} - e^{ -c d(m, m^ {\prime \prime}]}
\right]
& = 
\sum_m  \alpha_\ell (m)
e^{-c  d(m, m^\prime)} 
\left(
1 - e^{-c d(m^\prime, m^ {\prime \prime})}
\right) \\
&= 
\left(
1 - e^{-c d(m^\prime, m^ {\prime \prime})}
\right) 
\sum_m  \alpha_\ell (m)
e^{-c  d(m, m^\prime)} \\
&= \left(
1 - e^{-c d(m^\prime, m^ {\prime \prime})}
\right)  E[ e^{-c  d(m, m^\prime)} ]
\end{align*}
where $M \sim \alpha_\ell.$ That is, $\sum_m  \alpha_\ell (m)
e^{-c  d(m, m^\prime)} $ is the moment generating function of $d(M,m^\prime)$ (evaluated at c), where $M \sim \alpha_\ell.$ 
%
This implies that
\begin{align*}
&\sum_{i,j,\ell,m} \alpha_\ell (m) I(t_{ij\ell} \neq t^\prime_{ij\ell})
\left[
e^{-c  d(m, t_{ij\ell})} - e^{ -c d(m, t^\prime_{ij\ell}]}
\right]\\
&\quad\qquad\geq\sum_{i,j,\ell}
I(t_{ij\ell} \neq t^\prime_{ij\ell})
\left(
1 - e^{-c d(t_{ij\ell}, t^\prime_{ij\ell})}
\right) E[ e^{-c  d(m, t_{ij\ell})} ].
\end{align*}   
We have established that for any   $t_{ij\ell} \neq t^\prime_{ij\ell},$ that the lower bound grows as $c$ goes to~$\infty,$ at a rate determined by the moment generating function of the distances.

